DisParQ: Self-Supervised Part Concepts for Interpretable Vision Foundation Models

Concept-based vision models represent images through an intermediate layer of human-inspectable concepts, so what a model relies on can be traced to those concepts. However, those models are often limited to fixed categories or depend on language to define their concepts. We introduce DisParQ (Discrete Parts with Quantized attributes), a method that learns spatially grounded, discrete concept representations from a powerful frozen vision-only self-supervised backbone. It requires no class labels and no language supervision. Each image patch is assigned to exactly one concept from a learnable prototype dictionary, and only a sparse subset of concepts may activate per image. To capture how each concept varies across images (e.g., the type of a "wheel"), we learn continuous residuals alongside the concepts and then quantize them into discrete attributes. A spatial decoder reconstructs the backbone's representation from the concepts and attributes alone, so successful reconstruction means that the discrete representation preserves the backbone's information. We evaluate DisParQ across seven datasets, from general recognition (ImageNet, PartImageNet, Places) to fine-grained benchmarks (CUB, Cars, Dogs, Flowers). We show that DisParQ closely matches its frozen DINOv2 teacher on ImageNet linear probing (83.2% top-1), achieves higher concept consistency than language-aligned models, remains competitive on fine-grained recognition, and enables cross-category part-based retrieval.

==> repo/figures/user_study/violin_cars_data.tex <==
\path[fill=studyblue!35,draw=studyblue,line width=.45pt] (-0.127193,1.000000) -- (-0.128652,1.040404) -- (-0.129302,1.080808) -- (-0.129232,1.121212) -- (-0.128559,1.161616) -- (-0.127422,1.202020) -- (-0.125980,1.242424) -- (-0.124399,1.282828) -- (-0.122847,1.323232) -- (-0.121483,1.363636) -- (-0.120452,1.404040) -- (-0.119876,1.444444) -- (-0.119850,1.484848) -- (-0.120440,1.525253) -- (-0.121677,1.565657) -- (-0.123561,1.606061) -- (-0.126063,1.646465) -- (-0.129128,1.686869) -- (-0.132678,1.727273) -- (-0.136624,1.767677) -- (-0.140867,1.808081) -- (-0.145310,1.848485) -- (-0.149860,1.888889) -- (-0.154441,1.929293) -- (-0.158991,1.969697) -- (-0.163473,2.010101) -- (-0.167873,2.050505) -- (-0.172203,2.090909) -- (-0.176498,2.131313) -- (-0.180815,2.171717) -- (-0.185226,2.212121) -- (-0.189814,2.252525) -- (-0.194669,2.292929) -- (-0.199877,2.333333) -- (-0.205513,2.373737) -- (-0.211638,2.414141) -- (-0.218291,2.454545) -- (-0.225486,2.494949) -- (-0.233207,2.535354) -- (-0.241409,2.575758) -- (-0.250017,2.616162) -- (-0.258934,2.656566) -- (-0.268038,2.696970) -- (-0.277196,2.737374) -- (-0.286265,2.777778) -- (-0.295106,2.818182) -- (-0.303585,2.858586) -- (-0.311586,2.898990) -- (-0.319017,2.939394) -- (-0.325809,2.979798) -- (-0.331926,3.020202) -- (-0.337364,3.060606) -- (-0.342144,3.101010) -- (-0.346315,3.141414) -- (-0.349948,3.181818) -- (-0.353125,3.222222) -- (-0.355935,3.262626) -- (-0.358466,3.303030) -- (-0.360794,3.343434) -- (-0.362983,3.383838) -- (-0.365072,3.424242) -- (-0.367076,3.464646) -- (-0.368985,3.505051) -- (-0.370760,3.545455) -- (-0.372339,3.585859) -- (-0.373639,3.626263) -- (-0.374561,3.666667) -- (-0.375000,3.707071) -- (-0.374845,3.747475) -- (-0.373993,3.787879) -- (-0.372351,3.828283) -- (-0.369843,3.868687) -- (-0.366418,3.909091) -- (-0.362047,3.949495) -- (-0.356733,3.989899) -- (-0.350505,4.030303) -- (-0.343422,4.070707) -- (-0.335567,4.111111) -- (-0.327045,4.151515) -- (-0.317979,4.191919) -- (-0.308505,4.232323) -- (-0.298762,4.272727) -- (-0.288891,4.313131) -- (-0.279025,4.353535) -- (-0.269286,4.393939) -- (-0.259776,4.434343) -- (-0.250576,4.474747) -- (-0.241745,4.515152) -- (-0.233311,4.555556) -- (-0.225279,4.595960) -- (-0.217627,4.636364) -- (-0.210309,4.676768) -- (-0.203260,4.717172) -- (-0.196403,4.757576) -- (-0.189650,4.797980) -- (-0.182910,4.838384) -- (-0.176096,4.878788) -- (-0.169131,4.919192) -- (-0.161950,4.959596) -- (-0.154508,5.000000) -- (0.154508,5.000000) -- (0.161950,4.959596) -- (0.169131,4.919192) -- (0.176096,4.878788) -- (0.182910,4.838384) -- (0.189650,4.797980) -- (0.196403,4.757576) -- (0.203260,4.717172) -- (0.210309,4.676768) -- (0.217627,4.636364) -- (0.225279,4.595960) -- (0.233311,4.555556) -- (0.241745,4.515152) -- (0.250576,4.474747) -- (0.259776,4.434343) -- (0.269286,4.393939) -- (0.279025,4.353535) -- (0.288891,4.313131) -- (0.298762,4.272727) -- (0.308505,4.232323) -- (0.317979,4.191919) -- (0.327045,4.151515) -- (0.335567,4.111111) -- (0.343422,4.070707) -- (0.350505,4.030303) -- (0.356733,3.989899) -- (0.362047,3.949495) -- (0.366418,3.909091) -- (0.369843,3.868687) -- (0.372351,3.828283) -- (0.373993,3.787879) -- (0.374845,3.747475) -- (0.375000,3.707071) -- (0.374561,3.666667) -- (0.373639,3.626263) -- (0.372339,3.585859) -- (0.370760,3.545455) -- (0.368985,3.505051) -- (0.367076,3.464646) -- (0.365072,3.424242) -- (0.362983,3.383838) -- (0.360794,3.343434) -- (0.358466,3.303030) -- (0.355935,3.262626) -- (0.353125,3.222222) -- (0.349948,3.181818) -- (0.346315,3.141414) -- (0.342144,3.101010) -- (0.337364,3.060606) -- (0.331926,3.020202) -- (0.325809,2.979798) -- (0.319017,2.939394) -- (0.311586,2.898990) -- (0.303585,2.858586) -- (0.295106,2.818182) -- (0.286265,2.777778) -- (0.277196,2.737374) -- (0.268038,2.696970) -- (0.258934,2.656566) -- (0.250017,2.616162) -- (0.241409,2.575758) -- (0.233207,2.535354) -- (0.225486,2.494949) -- (0.218291,2.454545) -- (0.211638,2.414141) -- (0.205513,2.373737) -- (0.199877,2.333333) -- (0.194669,2.292929) -- (0.189814,2.252525) -- (0.185226,2.212121) -- (0.180815,2.171717) -- (0.176498,2.131313) -- (0.172203,2.090909) -- (0.167873,2.050505) -- (0.163473,2.010101) -- (0.158991,1.969697) -- (0.154441,1.929293) -- (0.149860,1.888889) -- (0.145310,1.848485) -- (0.140867,1.808081) -- (0.136624,1.767677) -- (0.132678,1.727273) -- (0.129128,1.686869) -- (0.126063,1.646465) -- (0.123561,1.606061) -- (0.121677,1.565657) -- (0.120440,1.525253) -- (0.119850,1.484848) -- (0.119876,1.444444) -- (0.120452,1.404040) -- (0.121483,1.363636) -- (0.122847,1.323232) -- (0.124399,1.282828) -- (0.125980,1.242424) -- (0.127422,1.202020) -- (0.128559,1.161616) -- (0.129232,1.121212) -- (0.129302,1.080808) -- (0.128652,1.040404) -- (0.127193,1.000000) -- cycle;
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.002837,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.108111,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.085402,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.107676,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.045160,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018402,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.078649,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.021792,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.011902,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.113386,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.060843,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009154,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.040864,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.069223,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.047233,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.011161,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.087830,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.023253,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.071171,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.057045,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.060088,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.052702,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.003554,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115377,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.110798,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.053950,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009894,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.053546,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.081444,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.112782,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.003856,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.092192,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.029638,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.066404,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027121,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.100151,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110498,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.006861,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.009759,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.105036,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.033919,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.084632,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.022306,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.057577,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.081572,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.002279,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.002613,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.060727,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.084499,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.076710,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.043989,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068903,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.074012,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.072567,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.074082,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.100427,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.085254,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.086708,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.090369,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.006742,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.054228,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.118298,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.034973,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.052778,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.080537,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.052349,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.068348,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.033440,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.073213,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.111281,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.083874,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.004269,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.094732,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018548,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.021480,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.114122,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.041630,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.100581,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.078438,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.092525,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.038485,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.061067,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.064444,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.069198,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.079506,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.104948,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.078117,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.080518,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.029965,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.043983,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.045921,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.077143,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.024899,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.118602,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.057001,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018915,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.094579,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.031958,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.028698,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.054071,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.036928,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.016506,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.088157,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.031712,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.074466,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.037969,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.010481,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072889,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.119074,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.061628,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.058352,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.102434,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.058127,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.063151,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.047494,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.089118,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.029703,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018979,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.039596,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.010577,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (0,2.583350) -- (0,4.000000);
\path[fill=white,draw=ink,line width=.45pt] (-0.045,3.225002) -- (0,3.335002) -- (0.045,3.225002) -- (0,3.115002) -- cycle;
\path[fill=studypeach!35,draw=studypeach,line width=.45pt] (0.871585,1.000000) -- (0.870203,1.040404) -- (0.869633,1.080808) -- (0.869767,1.121212) -- (0.870462,1.161616) -- (0.871548,1.202020) -- (0.872838,1.242424) -- (0.874130,1.282828) -- (0.875228,1.323232) -- (0.875938,1.363636) -- (0.876092,1.404040) -- (0.875542,1.444444) -- (0.874179,1.484848) -- (0.871926,1.525253) -- (0.868749,1.565657) -- (0.864653,1.606061) -- (0.859679,1.646465) -- (0.853900,1.686869) -- (0.847417,1.727273) -- (0.840348,1.767677) -- (0.832822,1.808081) -- (0.824970,1.848485) -- (0.816918,1.888889) -- (0.808778,1.929293) -- (0.800643,1.969697) -- (0.792584,2.010101) -- (0.784648,2.050505) -- (0.776855,2.090909) -- (0.769204,2.131313) -- (0.761673,2.171717) -- (0.754227,2.212121) -- (0.746821,2.252525) -- (0.739409,2.292929) -- (0.731949,2.333333) -- (0.724408,2.373737) -- (0.716767,2.414141) -- (0.709029,2.454545) -- (0.701214,2.494949) -- (0.693364,2.535354) -- (0.685544,2.575758) -- (0.677832,2.616162) -- (0.670321,2.656566) -- (0.663115,2.696970) -- (0.656317,2.737374) -- (0.650028,2.777778) -- (0.644341,2.818182) -- (0.639333,2.858586) -- (0.635062,2.898990) -- (0.631562,2.939394) -- (0.628842,2.979798) -- (0.626883,3.020202) -- (0.625639,3.060606) -- (0.625042,3.101010) -- (0.625000,3.141414) -- (0.625403,3.181818) -- (0.626131,3.222222) -- (0.627057,3.262626) -- (0.628056,3.303030) -- (0.629012,3.343434) -- (0.629822,3.383838) -- (0.630405,3.424242) -- (0.630707,3.464646) -- (0.630701,3.505051) -- (0.630396,3.545455) -- (0.629833,3.585859) -- (0.629085,3.626263) -- (0.628254,3.666667) -- (0.627467,3.707071) -- (0.626869,3.747475) -- (0.626618,3.787879) -- (0.626871,3.828283) -- (0.627781,3.868687) -- (0.629485,3.909091) -- (0.632097,3.949495) -- (0.635702,3.989899) -- (0.640349,4.030303) -- (0.646047,4.070707) -- (0.652767,4.111111) -- (0.660439,4.151515) -- (0.668958,4.191919) -- (0.678187,4.232323) -- (0.687966,4.272727) -- (0.698119,4.313131) -- (0.708467,4.353535) -- (0.718830,4.393939) -- (0.729044,4.434343) -- (0.738966,4.474747) -- (0.748481,4.515152) -- (0.757509,4.555556) -- (0.766007,4.595960) -- (0.773969,4.636364) -- (0.781426,4.676768) -- (0.788443,4.717172) -- (0.795111,4.757576) -- (0.801542,4.797980) -- (0.807858,4.838384) -- (0.814185,4.878788) -- (0.820642,4.919192) -- (0.827337,4.959596) -- (0.834354,5.000000) -- (1.165646,5.000000) -- (1.172663,4.959596) -- (1.179358,4.919192) -- (1.185815,4.878788) -- (1.192142,4.838384) -- (1.198458,4.797980) -- (1.204889,4.757576) -- (1.211557,4.717172) -- (1.218574,4.676768) -- (1.226031,4.636364) -- (1.233993,4.595960) -- (1.242491,4.555556) -- (1.251519,4.515152) -- (1.261034,4.474747) -- (1.270956,4.434343) -- (1.281170,4.393939) -- (1.291533,4.353535) -- (1.301881,4.313131) -- (1.312034,4.272727) -- (1.321813,4.232323) -- (1.331042,4.191919) -- (1.339561,4.151515) -- (1.347233,4.111111) -- (1.353953,4.070707) -- (1.359651,4.030303) -- (1.364298,3.989899) -- (1.367903,3.949495) -- (1.370515,3.909091) -- (1.372219,3.868687) -- (1.373129,3.828283) -- (1.373382,3.787879) -- (1.373131,3.747475) -- (1.372533,3.707071) -- (1.371746,3.666667) -- (1.370915,3.626263) -- (1.370167,3.585859) -- (1.369604,3.545455) -- (1.369299,3.505051) -- (1.369293,3.464646) -- (1.369595,3.424242) -- (1.370178,3.383838) -- (1.370988,3.343434) -- (1.371944,3.303030) -- (1.372943,3.262626) -- (1.373869,3.222222) -- (1.374597,3.181818) -- (1.375000,3.141414) -- (1.374958,3.101010) -- (1.374361,3.060606) -- (1.373117,3.020202) -- (1.371158,2.979798) -- (1.368438,2.939394) -- (1.364938,2.898990) -- (1.360667,2.858586) -- (1.355659,2.818182) -- (1.349972,2.777778) -- (1.343683,2.737374) -- (1.336885,2.696970) -- (1.329679,2.656566) -- (1.322168,2.616162) -- (1.314456,2.575758) -- (1.306636,2.535354) -- (1.298786,2.494949) -- (1.290971,2.454545) -- (1.283233,2.414141) -- (1.275592,2.373737) -- (1.268051,2.333333) -- (1.260591,2.292929) -- (1.253179,2.252525) -- (1.245773,2.212121) -- (1.238327,2.171717) -- (1.230796,2.131313) -- (1.223145,2.090909) -- (1.215352,2.050505) -- (1.207416,2.010101) -- (1.199357,1.969697) -- (1.191222,1.929293) -- (1.183082,1.888889) -- (1.175030,1.848485) -- (1.167178,1.808081) -- (1.159652,1.767677) -- (1.152583,1.727273) -- (1.146100,1.686869) -- (1.140321,1.646465) -- (1.135347,1.606061) -- (1.131251,1.565657) -- (1.128074,1.525253) -- (1.125821,1.484848) -- (1.124458,1.444444) -- (1.123908,1.404040) -- (1.124062,1.363636) -- (1.124772,1.323232) -- (1.125870,1.282828) -- (1.127162,1.242424) -- (1.128452,1.202020) -- (1.129538,1.161616) -- (1.130233,1.121212) -- (1.130367,1.080808) -- (1.129797,1.040404) -- (1.128415,1.000000) -- cycle;
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.002837,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.108111,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.914598,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.107676,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.954840,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981598,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.078649,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.978208,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.011902,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.886614,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.060843,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009154,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.959136,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.069223,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.952767,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.988839,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.912170,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.976747,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.928829,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.942955,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.060088,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.947298,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.996446,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115377,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.110798,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.053950,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009894,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.946454,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.918556,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.112782,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.003856,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.907808,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.029638,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.066404,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027121,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.100151,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889502,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.006861,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.990241,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.894964,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.033919,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.084632,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.022306,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.942423,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.081572,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.002279,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.002613,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.060727,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.915501,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.076710,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.043989,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068903,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.925988,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.072567,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.925918,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.899573,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.085254,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.086708,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.090369,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.993258,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.945772,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.881702,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.034973,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.052778,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.080537,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.947651,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.931652,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.033440,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.073213,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.111281,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.916126,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.995731,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.094732,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981452,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.021480,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.885878,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.041630,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.100581,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.078438,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.092525,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.038485,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.938933,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.064444,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.930802,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.079506,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.895052,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.078117,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.919482,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.970035,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.956017,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.045921,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.922857,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.975101,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.881398,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.942999,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981085,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.905421,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.031958,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.971302,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.054071,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.036928,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.983494,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.088157,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.031712,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.074466,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.962031,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.010481,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927111,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.119074,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.938372,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.941648,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.897566,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.941873,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.063151,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.047494,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.910882,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.970297,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981021,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.039596,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.989423,4.333300) circle[radius=.65pt];
\draw[ink,line width=2pt] (1,2.583350) -- (1,4.000000);
\path[fill=white,draw=ink,line width=.45pt] (0.955,3.194444) -- (1,3.304444) -- (1.045,3.194444) -- (1,3.084444) -- cycle;
\path[fill=studygray!35,draw=studygray,line width=.45pt] (1.800570,1.000000) -- (1.799233,1.040404) -- (1.799219,1.080808) -- (1.800431,1.121212) -- (1.802731,1.161616) -- (1.805951,1.202020) -- (1.809892,1.242424) -- (1.814342,1.282828) -- (1.819076,1.323232) -- (1.823872,1.363636) -- (1.828514,1.404040) -- (1.832805,1.444444) -- (1.836569,1.484848) -- (1.839662,1.525253) -- (1.841969,1.565657) -- (1.843408,1.606061) -- (1.843933,1.646465) -- (1.843527,1.686869) -- (1.842202,1.727273) -- (1.839995,1.767677) -- (1.836960,1.808081) -- (1.833166,1.848485) -- (1.828689,1.888889) -- (1.823605,1.929293) -- (1.817990,1.969697) -- (1.811913,2.010101) -- (1.805431,2.050505) -- (1.798594,2.090909) -- (1.791435,2.131313) -- (1.783980,2.171717) -- (1.776242,2.212121) -- (1.768229,2.252525) -- (1.759945,2.292929) -- (1.751395,2.333333) -- (1.742587,2.373737) -- (1.733539,2.414141) -- (1.724280,2.454545) -- (1.714855,2.494949) -- (1.705328,2.535354) -- (1.695778,2.575758) -- (1.686306,2.616162) -- (1.677029,2.656566) -- (1.668077,2.696970) -- (1.659593,2.737374) -- (1.651725,2.777778) -- (1.644622,2.818182) -- (1.638428,2.858586) -- (1.633274,2.898990) -- (1.629276,2.939394) -- (1.626525,2.979798) -- (1.625089,3.020202) -- (1.625000,3.060606) -- (1.626263,3.101010) -- (1.628846,3.141414) -- (1.632687,3.181818) -- (1.637694,3.222222) -- (1.643747,3.262626) -- (1.650707,3.303030) -- (1.658416,3.343434) -- (1.666707,3.383838) -- (1.675410,3.424242) -- (1.684357,3.464646) -- (1.693388,3.505051) -- (1.702357,3.545455) -- (1.711136,3.585859) -- (1.719616,3.626263) -- (1.727713,3.666667) -- (1.735367,3.707071) -- (1.742539,3.747475) -- (1.749216,3.787879) -- (1.755400,3.828283) -- (1.761114,3.868687) -- (1.766391,3.909091) -- (1.771277,3.949495) -- (1.775820,3.989899) -- (1.780074,4.030303) -- (1.784088,4.070707) -- (1.787912,4.111111) -- (1.791587,4.151515) -- (1.795151,4.191919) -- (1.798633,4.232323) -- (1.802056,4.272727) -- (1.805439,4.313131) -- (1.808796,4.353535) -- (1.812137,4.393939) -- (1.815474,4.434343) -- (1.818818,4.474747) -- (1.822185,4.515152) -- (1.825591,4.555556) -- (1.829060,4.595960) -- (1.832619,4.636364) -- (1.836297,4.676768) -- (1.840128,4.717172) -- (1.844147,4.757576) -- (1.848387,4.797980) -- (1.852881,4.838384) -- (1.857653,4.878788) -- (1.862724,4.919192) -- (1.868102,4.959596) -- (1.873787,5.000000) -- (2.126213,5.000000) -- (2.131898,4.959596) -- (2.137276,4.919192) -- (2.142347,4.878788) -- (2.147119,4.838384) -- (2.151613,4.797980) -- (2.155853,4.757576) -- (2.159872,4.717172) -- (2.163703,4.676768) -- (2.167381,4.636364) -- (2.170940,4.595960) -- (2.174409,4.555556) -- (2.177815,4.515152) -- (2.181182,4.474747) -- (2.184526,4.434343) -- (2.187863,4.393939) -- (2.191204,4.353535) -- (2.194561,4.313131) -- (2.197944,4.272727) -- (2.201367,4.232323) -- (2.204849,4.191919) -- (2.208413,4.151515) -- (2.212088,4.111111) -- (2.215912,4.070707) -- (2.219926,4.030303) -- (2.224180,3.989899) -- (2.228723,3.949495) -- (2.233609,3.909091) -- (2.238886,3.868687) -- (2.244600,3.828283) -- (2.250784,3.787879) -- (2.257461,3.747475) -- (2.264633,3.707071) -- (2.272287,3.666667) -- (2.280384,3.626263) -- (2.288864,3.585859) -- (2.297643,3.545455) -- (2.306612,3.505051) -- (2.315643,3.464646) -- (2.324590,3.424242) -- (2.333293,3.383838) -- (2.341584,3.343434) -- (2.349293,3.303030) -- (2.356253,3.262626) -- (2.362306,3.222222) -- (2.367313,3.181818) -- (2.371154,3.141414) -- (2.373737,3.101010) -- (2.375000,3.060606) -- (2.374911,3.020202) -- (2.373475,2.979798) -- (2.370724,2.939394) -- (2.366726,2.898990) -- (2.361572,2.858586) -- (2.355378,2.818182) -- (2.348275,2.777778) -- (2.340407,2.737374) -- (2.331923,2.696970) -- (2.322971,2.656566) -- (2.313694,2.616162) -- (2.304222,2.575758) -- (2.294672,2.535354) -- (2.285145,2.494949) -- (2.275720,2.454545) -- (2.266461,2.414141) -- (2.257413,2.373737) -- (2.248605,2.333333) -- (2.240055,2.292929) -- (2.231771,2.252525) -- (2.223758,2.212121) -- (2.216020,2.171717) -- (2.208565,2.131313) -- (2.201406,2.090909) -- (2.194569,2.050505) -- (2.188087,2.010101) -- (2.182010,1.969697) -- (2.176395,1.929293) -- (2.171311,1.888889) -- (2.166834,1.848485) -- (2.163040,1.808081) -- (2.160005,1.767677) -- (2.157798,1.727273) -- (2.156473,1.686869) -- (2.156067,1.646465) -- (2.156592,1.606061) -- (2.158031,1.565657) -- (2.160338,1.525253) -- (2.163431,1.484848) -- (2.167195,1.444444) -- (2.171486,1.404040) -- (2.176128,1.363636) -- (2.180924,1.323232) -- (2.185658,1.282828) -- (2.190108,1.242424) -- (2.194049,1.202020) -- (2.197269,1.161616) -- (2.199569,1.121212) -- (2.200781,1.080808) -- (2.200767,1.040404) -- (2.199430,1.000000) -- cycle;
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.002837,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.108111,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.914598,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.107676,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.954840,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981598,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.078649,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.978208,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.011902,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.886614,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.060843,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009154,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.959136,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.069223,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.952767,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.988839,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.912170,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.976747,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.928829,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.942955,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.060088,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.947298,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.996446,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115377,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.110798,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.053950,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009894,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.946454,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.918556,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.112782,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.003856,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.907808,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.029638,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.066404,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027121,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.100151,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889502,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.006861,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.990241,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.894964,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.033919,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.084632,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.022306,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.942423,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.081572,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.002279,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.002613,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.060727,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.915501,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.076710,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.043989,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068903,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.925988,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.072567,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.925918,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.899573,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.085254,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.086708,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.090369,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.993258,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.945772,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.881702,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.034973,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.052778,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.080537,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.947651,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.931652,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.033440,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.073213,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.111281,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.916126,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.995731,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.094732,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981452,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.021480,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.885878,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.041630,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.100581,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.078438,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.092525,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.038485,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.938933,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.064444,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.930802,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.079506,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.895052,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.078117,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.919482,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.970035,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.956017,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.045921,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.922857,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.975101,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.881398,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.942999,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981085,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.905421,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.031958,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.971302,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.054071,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.036928,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.983494,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.088157,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.031712,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.074466,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.962031,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.010481,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927111,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.119074,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.938372,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.941648,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.897566,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.941873,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.063151,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.047494,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.910882,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.970297,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981021,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.039596,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.989423,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (2,2.000000) -- (2,3.750025);
\path[fill=white,draw=ink,line width=.45pt] (1.955,2.899997) -- (2,3.009997) -- (2.045,2.899997) -- (2,2.789997) -- cycle;


==> repo/figures/user_study/violin_cars_stats.tex <==
\draw[ink,line width=.45pt] (0,5.13) -- (0,5.20) -- (2,5.20) -- (2,5.13);
\node[anchor=south] at (1,5.20) {$^{*}$};


==> repo/figures/user_study/violin_cub_data.tex <==
\path[fill=studyblue!35,draw=studyblue,line width=.45pt] (-0.102490,1.000000) -- (-0.103391,1.040404) -- (-0.103502,1.080808) -- (-0.102854,1.121212) -- (-0.101501,1.161616) -- (-0.099516,1.202020) -- (-0.096992,1.242424) -- (-0.094038,1.282828) -- (-0.090771,1.323232) -- (-0.087317,1.363636) -- (-0.083801,1.404040) -- (-0.080349,1.444444) -- (-0.077076,1.484848) -- (-0.074091,1.525253) -- (-0.071488,1.565657) -- (-0.069350,1.606061) -- (-0.067740,1.646465) -- (-0.066709,1.686869) -- (-0.066291,1.727273) -- (-0.066507,1.767677) -- (-0.067364,1.808081) -- (-0.068857,1.848485) -- (-0.070973,1.888889) -- (-0.073693,1.929293) -- (-0.076989,1.969697) -- (-0.080833,2.010101) -- (-0.085192,2.050505) -- (-0.090031,2.090909) -- (-0.095316,2.131313) -- (-0.101009,2.171717) -- (-0.107074,2.212121) -- (-0.113472,2.252525) -- (-0.120159,2.292929) -- (-0.127091,2.333333) -- (-0.134219,2.373737) -- (-0.141490,2.414141) -- (-0.148848,2.454545) -- (-0.156230,2.494949) -- (-0.163573,2.535354) -- (-0.170810,2.575758) -- (-0.177876,2.616162) -- (-0.184708,2.656566) -- (-0.191246,2.696970) -- (-0.197443,2.737374) -- (-0.203261,2.777778) -- (-0.208675,2.818182) -- (-0.213681,2.858586) -- (-0.218292,2.898990) -- (-0.222540,2.939394) -- (-0.226482,2.979798) -- (-0.230191,3.020202) -- (-0.233759,3.060606) -- (-0.237292,3.101010) -- (-0.240907,3.141414) -- (-0.244722,3.181818) -- (-0.248856,3.222222) -- (-0.253418,3.262626) -- (-0.258500,3.303030) -- (-0.264173,3.343434) -- (-0.270478,3.383838) -- (-0.277425,3.424242) -- (-0.284986,3.464646) -- (-0.293096,3.505051) -- (-0.301652,3.545455) -- (-0.310516,3.585859) -- (-0.319522,3.626263) -- (-0.328476,3.666667) -- (-0.337172,3.707071) -- (-0.345397,3.747475) -- (-0.352940,3.787879) -- (-0.359605,3.828283) -- (-0.365220,3.868687) -- (-0.369645,3.909091) -- (-0.372779,3.949495) -- (-0.374567,3.989899) -- (-0.375000,4.030303) -- (-0.374117,4.070707) -- (-0.372001,4.111111) -- (-0.368777,4.151515) -- (-0.364599,4.191919) -- (-0.359647,4.232323) -- (-0.354113,4.272727) -- (-0.348191,4.313131) -- (-0.342064,4.353535) -- (-0.335898,4.393939) -- (-0.329829,4.434343) -- (-0.323959,4.474747) -- (-0.318346,4.515152) -- (-0.313010,4.555556) -- (-0.307926,4.595960) -- (-0.303029,4.636364) -- (-0.298223,4.676768) -- (-0.293381,4.717172) -- (-0.288362,4.757576) -- (-0.283014,4.797980) -- (-0.277189,4.838384) -- (-0.270749,4.878788) -- (-0.263578,4.919192) -- (-0.255587,4.959596) -- (-0.246720,5.000000) -- (0.246720,5.000000) -- (0.255587,4.959596) -- (0.263578,4.919192) -- (0.270749,4.878788) -- (0.277189,4.838384) -- (0.283014,4.797980) -- (0.288362,4.757576) -- (0.293381,4.717172) -- (0.298223,4.676768) -- (0.303029,4.636364) -- (0.307926,4.595960) -- (0.313010,4.555556) -- (0.318346,4.515152) -- (0.323959,4.474747) -- (0.329829,4.434343) -- (0.335898,4.393939) -- (0.342064,4.353535) -- (0.348191,4.313131) -- (0.354113,4.272727) -- (0.359647,4.232323) -- (0.364599,4.191919) -- (0.368777,4.151515) -- (0.372001,4.111111) -- (0.374117,4.070707) -- (0.375000,4.030303) -- (0.374567,3.989899) -- (0.372779,3.949495) -- (0.369645,3.909091) -- (0.365220,3.868687) -- (0.359605,3.828283) -- (0.352940,3.787879) -- (0.345397,3.747475) -- (0.337172,3.707071) -- (0.328476,3.666667) -- (0.319522,3.626263) -- (0.310516,3.585859) -- (0.301652,3.545455) -- (0.293096,3.505051) -- (0.284986,3.464646) -- (0.277425,3.424242) -- (0.270478,3.383838) -- (0.264173,3.343434) -- (0.258500,3.303030) -- (0.253418,3.262626) -- (0.248856,3.222222) -- (0.244722,3.181818) -- (0.240907,3.141414) -- (0.237292,3.101010) -- (0.233759,3.060606) -- (0.230191,3.020202) -- (0.226482,2.979798) -- (0.222540,2.939394) -- (0.218292,2.898990) -- (0.213681,2.858586) -- (0.208675,2.818182) -- (0.203261,2.777778) -- (0.197443,2.737374) -- (0.191246,2.696970) -- (0.184708,2.656566) -- (0.177876,2.616162) -- (0.170810,2.575758) -- (0.163573,2.535354) -- (0.156230,2.494949) -- (0.148848,2.454545) -- (0.141490,2.414141) -- (0.134219,2.373737) -- (0.127091,2.333333) -- (0.120159,2.292929) -- (0.113472,2.252525) -- (0.107074,2.212121) -- (0.101009,2.171717) -- (0.095316,2.131313) -- (0.090031,2.090909) -- (0.085192,2.050505) -- (0.080833,2.010101) -- (0.076989,1.969697) -- (0.073693,1.929293) -- (0.070973,1.888889) -- (0.068857,1.848485) -- (0.067364,1.808081) -- (0.066507,1.767677) -- (0.066291,1.727273) -- (0.066709,1.686869) -- (0.067740,1.646465) -- (0.069350,1.606061) -- (0.071488,1.565657) -- (0.074091,1.525253) -- (0.077076,1.484848) -- (0.080349,1.444444) -- (0.083801,1.404040) -- (0.087317,1.363636) -- (0.090771,1.323232) -- (0.094038,1.282828) -- (0.096992,1.242424) -- (0.099516,1.202020) -- (0.101501,1.161616) -- (0.102854,1.121212) -- (0.103502,1.080808) -- (0.103391,1.040404) -- (0.102490,1.000000) -- cycle;
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.032871,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.055251,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110166,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116033,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.075185,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.099061,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.025593,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055079,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.010470,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.104417,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.075805,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.119343,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.085777,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.111939,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055117,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.077843,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.087163,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009951,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048069,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018555,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.113203,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.090172,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.040950,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.035325,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027692,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.027917,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.119330,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115400,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.044530,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.036110,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.045227,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026659,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.087577,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.053157,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.006085,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.045542,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.003400,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093477,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.104170,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.034129,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.017167,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.042751,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.022632,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.038901,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026011,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093666,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.065482,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.029565,1.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.099836,1.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068904,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.062551,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.090356,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.105944,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.039332,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.083933,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.011919,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.071118,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.064646,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.107515,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.022908,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072357,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.098219,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.019280,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048313,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.041279,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072116,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.106107,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.032374,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.094681,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.030986,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102517,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.014309,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.109102,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.000025,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.017945,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.118823,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.107746,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.009589,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.000619,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.007035,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068589,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.020483,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.056276,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.050674,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.103694,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.092416,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.054964,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102582,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.112302,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116470,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.087274,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.109730,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.084297,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.113431,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093585,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.077370,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.004803,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.064230,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.072451,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.101647,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.056129,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009344,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.013739,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.103444,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110277,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055681,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027450,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.113192,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.052613,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116162,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.061908,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.003062,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102985,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.104140,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.081916,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.103994,5.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (0,3.000000) -- (0,4.333300);
\path[fill=white,draw=ink,line width=.45pt] (-0.045,3.566668) -- (0,3.676668) -- (0.045,3.566668) -- (0,3.456668) -- cycle;
\path[fill=studypeach!35,draw=studypeach,line width=.45pt] (0.872721,1.000000) -- (0.871872,1.040404) -- (0.871891,1.080808) -- (0.872674,1.121212) -- (0.874086,1.161616) -- (0.875962,1.202020) -- (0.878115,1.242424) -- (0.880350,1.282828) -- (0.882464,1.323232) -- (0.884264,1.363636) -- (0.885571,1.404040) -- (0.886229,1.444444) -- (0.886114,1.484848) -- (0.885137,1.525253) -- (0.883245,1.565657) -- (0.880427,1.606061) -- (0.876711,1.646465) -- (0.872158,1.686869) -- (0.866860,1.727273) -- (0.860935,1.767677) -- (0.854515,1.808081) -- (0.847742,1.848485) -- (0.840759,1.888889) -- (0.833700,1.929293) -- (0.826687,1.969697) -- (0.819821,2.010101) -- (0.813177,2.050505) -- (0.806805,2.090909) -- (0.800726,2.131313) -- (0.794935,2.171717) -- (0.789400,2.212121) -- (0.784069,2.252525) -- (0.778877,2.292929) -- (0.773746,2.333333) -- (0.768596,2.373737) -- (0.763351,2.414141) -- (0.757943,2.454545) -- (0.752318,2.494949) -- (0.746442,2.535354) -- (0.740301,2.575758) -- (0.733903,2.616162) -- (0.727278,2.656566) -- (0.720477,2.696970) -- (0.713565,2.737374) -- (0.706622,2.777778) -- (0.699735,2.818182) -- (0.692989,2.858586) -- (0.686469,2.898990) -- (0.680249,2.939394) -- (0.674390,2.979798) -- (0.668937,3.020202) -- (0.663913,3.060606) -- (0.659327,3.101010) -- (0.655167,3.141414) -- (0.651407,3.181818) -- (0.648008,3.222222) -- (0.644924,3.262626) -- (0.642108,3.303030) -- (0.639515,3.343434) -- (0.637107,3.383838) -- (0.634859,3.424242) -- (0.632763,3.464646) -- (0.630825,3.505051) -- (0.629072,3.545455) -- (0.627549,3.585859) -- (0.626314,3.626263) -- (0.625438,3.666667) -- (0.625000,3.707071) -- (0.625082,3.747475) -- (0.625762,3.787879) -- (0.627110,3.828283) -- (0.629182,3.868687) -- (0.632016,3.909091) -- (0.635628,3.949495) -- (0.640014,3.989899) -- (0.645142,4.030303) -- (0.650960,4.070707) -- (0.657395,4.111111) -- (0.664356,4.151515) -- (0.671742,4.191919) -- (0.679443,4.232323) -- (0.687351,4.272727) -- (0.695362,4.313131) -- (0.703383,4.353535) -- (0.711336,4.393939) -- (0.719164,4.434343) -- (0.726830,4.474747) -- (0.734322,4.515152) -- (0.741649,4.555556) -- (0.748843,4.595960) -- (0.755951,4.636364) -- (0.763038,4.676768) -- (0.770175,4.717172) -- (0.777437,4.757576) -- (0.784898,4.797980) -- (0.792625,4.838384) -- (0.800672,4.878788) -- (0.809077,4.919192) -- (0.817860,4.959596) -- (0.827020,5.000000) -- (1.172980,5.000000) -- (1.182140,4.959596) -- (1.190923,4.919192) -- (1.199328,4.878788) -- (1.207375,4.838384) -- (1.215102,4.797980) -- (1.222563,4.757576) -- (1.229825,4.717172) -- (1.236962,4.676768) -- (1.244049,4.636364) -- (1.251157,4.595960) -- (1.258351,4.555556) -- (1.265678,4.515152) -- (1.273170,4.474747) -- (1.280836,4.434343) -- (1.288664,4.393939) -- (1.296617,4.353535) -- (1.304638,4.313131) -- (1.312649,4.272727) -- (1.320557,4.232323) -- (1.328258,4.191919) -- (1.335644,4.151515) -- (1.342605,4.111111) -- (1.349040,4.070707) -- (1.354858,4.030303) -- (1.359986,3.989899) -- (1.364372,3.949495) -- (1.367984,3.909091) -- (1.370818,3.868687) -- (1.372890,3.828283) -- (1.374238,3.787879) -- (1.374918,3.747475) -- (1.375000,3.707071) -- (1.374562,3.666667) -- (1.373686,3.626263) -- (1.372451,3.585859) -- (1.370928,3.545455) -- (1.369175,3.505051) -- (1.367237,3.464646) -- (1.365141,3.424242) -- (1.362893,3.383838) -- (1.360485,3.343434) -- (1.357892,3.303030) -- (1.355076,3.262626) -- (1.351992,3.222222) -- (1.348593,3.181818) -- (1.344833,3.141414) -- (1.340673,3.101010) -- (1.336087,3.060606) -- (1.331063,3.020202) -- (1.325610,2.979798) -- (1.319751,2.939394) -- (1.313531,2.898990) -- (1.307011,2.858586) -- (1.300265,2.818182) -- (1.293378,2.777778) -- (1.286435,2.737374) -- (1.279523,2.696970) -- (1.272722,2.656566) -- (1.266097,2.616162) -- (1.259699,2.575758) -- (1.253558,2.535354) -- (1.247682,2.494949) -- (1.242057,2.454545) -- (1.236649,2.414141) -- (1.231404,2.373737) -- (1.226254,2.333333) -- (1.221123,2.292929) -- (1.215931,2.252525) -- (1.210600,2.212121) -- (1.205065,2.171717) -- (1.199274,2.131313) -- (1.193195,2.090909) -- (1.186823,2.050505) -- (1.180179,2.010101) -- (1.173313,1.969697) -- (1.166300,1.929293) -- (1.159241,1.888889) -- (1.152258,1.848485) -- (1.145485,1.808081) -- (1.139065,1.767677) -- (1.133140,1.727273) -- (1.127842,1.686869) -- (1.123289,1.646465) -- (1.119573,1.606061) -- (1.116755,1.565657) -- (1.114863,1.525253) -- (1.113886,1.484848) -- (1.113771,1.444444) -- (1.114429,1.404040) -- (1.115736,1.363636) -- (1.117536,1.323232) -- (1.119650,1.282828) -- (1.121885,1.242424) -- (1.124038,1.202020) -- (1.125914,1.161616) -- (1.127326,1.121212) -- (1.128109,1.080808) -- (1.128128,1.040404) -- (1.127279,1.000000) -- cycle;
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.032871,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.944749,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889834,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883967,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.075185,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.099061,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.025593,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055079,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.010470,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.104417,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.075805,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.880657,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.085777,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.888061,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055117,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.922157,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.087163,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009951,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951931,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981445,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.886797,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.909828,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.040950,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.035325,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027692,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.972083,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.119330,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115400,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.044530,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.036110,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.045227,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973341,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.912423,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.053157,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.006085,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.954458,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.996600,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093477,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.104170,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.965871,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.017167,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.957249,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.022632,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.961099,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973989,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093666,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.934518,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.029565,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.900164,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068904,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.937449,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.090356,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.894056,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.960668,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.916067,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.988081,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.071118,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.935354,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.892485,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.977092,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927643,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.901781,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.019280,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951687,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.041279,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927884,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.106107,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.967626,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.905319,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.030986,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102517,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.985691,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.109102,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.999975,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.982055,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.118823,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.107746,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.990411,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.999381,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.007035,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068589,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.979517,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.056276,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.050674,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.103694,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.907584,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.054964,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102582,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.112302,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883530,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.087274,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.109730,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.915703,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.113431,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093585,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.077370,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.995197,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.935770,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.072451,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.101647,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.943871,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009344,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.986261,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.103444,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889723,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055681,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027450,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.886808,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.052613,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883838,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.061908,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.003062,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102985,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.895860,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.081916,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.896006,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (1,2.333300) -- (1,4.000000);
\path[fill=white,draw=ink,line width=.45pt] (0.955,3.241667) -- (1,3.351667) -- (1.045,3.241667) -- (1,3.131667) -- cycle;
\path[fill=studygray!35,draw=studygray,line width=.45pt] (1.840743,1.000000) -- (1.835887,1.040404) -- (1.831546,1.080808) -- (1.827673,1.121212) -- (1.824207,1.161616) -- (1.821072,1.202020) -- (1.818184,1.242424) -- (1.815452,1.282828) -- (1.812785,1.323232) -- (1.810096,1.363636) -- (1.807303,1.404040) -- (1.804337,1.444444) -- (1.801141,1.484848) -- (1.797673,1.525253) -- (1.793904,1.565657) -- (1.789820,1.606061) -- (1.785422,1.646465) -- (1.780720,1.686869) -- (1.775734,1.727273) -- (1.770489,1.767677) -- (1.765014,1.808081) -- (1.759338,1.848485) -- (1.753489,1.888889) -- (1.747491,1.929293) -- (1.741364,1.969697) -- (1.735121,2.010101) -- (1.728773,2.050505) -- (1.722326,2.090909) -- (1.715784,2.131313) -- (1.709151,2.171717) -- (1.702435,2.212121) -- (1.695649,2.252525) -- (1.688812,2.292929) -- (1.681956,2.333333) -- (1.675122,2.373737) -- (1.668367,2.414141) -- (1.661760,2.454545) -- (1.655385,2.494949) -- (1.649335,2.535354) -- (1.643713,2.575758) -- (1.638631,2.616162) -- (1.634198,2.656566) -- (1.630525,2.696970) -- (1.627711,2.737374) -- (1.625846,2.777778) -- (1.625000,2.818182) -- (1.625222,2.858586) -- (1.626533,2.898990) -- (1.628929,2.939394) -- (1.632374,2.979798) -- (1.636801,3.020202) -- (1.642115,3.060606) -- (1.648195,3.101010) -- (1.654899,3.141414) -- (1.662067,3.181818) -- (1.669529,3.222222) -- (1.677112,3.262626) -- (1.684645,3.303030) -- (1.691969,3.343434) -- (1.698941,3.383838) -- (1.705441,3.424242) -- (1.711377,3.464646) -- (1.716685,3.505051) -- (1.721336,3.545455) -- (1.725330,3.585859) -- (1.728697,3.626263) -- (1.731495,3.666667) -- (1.733801,3.707071) -- (1.735711,3.747475) -- (1.737327,3.787879) -- (1.738755,3.828283) -- (1.740097,3.868687) -- (1.741442,3.909091) -- (1.742866,3.949495) -- (1.744424,3.989899) -- (1.746146,4.030303) -- (1.748042,4.070707) -- (1.750095,4.111111) -- (1.752272,4.151515) -- (1.754519,4.191919) -- (1.756773,4.232323) -- (1.758962,4.272727) -- (1.761017,4.313131) -- (1.762876,4.353535) -- (1.764487,4.393939) -- (1.765820,4.434343) -- (1.766865,4.474747) -- (1.767640,4.515152) -- (1.768186,4.555556) -- (1.768573,4.595960) -- (1.768894,4.636364) -- (1.769263,4.676768) -- (1.769806,4.717172) -- (1.770663,4.757576) -- (1.771970,4.797980) -- (1.773863,4.838384) -- (1.776463,4.878788) -- (1.779873,4.919192) -- (1.784171,4.959596) -- (1.789409,5.000000) -- (2.210591,5.000000) -- (2.215829,4.959596) -- (2.220127,4.919192) -- (2.223537,4.878788) -- (2.226137,4.838384) -- (2.228030,4.797980) -- (2.229337,4.757576) -- (2.230194,4.717172) -- (2.230737,4.676768) -- (2.231106,4.636364) -- (2.231427,4.595960) -- (2.231814,4.555556) -- (2.232360,4.515152) -- (2.233135,4.474747) -- (2.234180,4.434343) -- (2.235513,4.393939) -- (2.237124,4.353535) -- (2.238983,4.313131) -- (2.241038,4.272727) -- (2.243227,4.232323) -- (2.245481,4.191919) -- (2.247728,4.151515) -- (2.249905,4.111111) -- (2.251958,4.070707) -- (2.253854,4.030303) -- (2.255576,3.989899) -- (2.257134,3.949495) -- (2.258558,3.909091) -- (2.259903,3.868687) -- (2.261245,3.828283) -- (2.262673,3.787879) -- (2.264289,3.747475) -- (2.266199,3.707071) -- (2.268505,3.666667) -- (2.271303,3.626263) -- (2.274670,3.585859) -- (2.278664,3.545455) -- (2.283315,3.505051) -- (2.288623,3.464646) -- (2.294559,3.424242) -- (2.301059,3.383838) -- (2.308031,3.343434) -- (2.315355,3.303030) -- (2.322888,3.262626) -- (2.330471,3.222222) -- (2.337933,3.181818) -- (2.345101,3.141414) -- (2.351805,3.101010) -- (2.357885,3.060606) -- (2.363199,3.020202) -- (2.367626,2.979798) -- (2.371071,2.939394) -- (2.373467,2.898990) -- (2.374778,2.858586) -- (2.375000,2.818182) -- (2.374154,2.777778) -- (2.372289,2.737374) -- (2.369475,2.696970) -- (2.365802,2.656566) -- (2.361369,2.616162) -- (2.356287,2.575758) -- (2.350665,2.535354) -- (2.344615,2.494949) -- (2.338240,2.454545) -- (2.331633,2.414141) -- (2.324878,2.373737) -- (2.318044,2.333333) -- (2.311188,2.292929) -- (2.304351,2.252525) -- (2.297565,2.212121) -- (2.290849,2.171717) -- (2.284216,2.131313) -- (2.277674,2.090909) -- (2.271227,2.050505) -- (2.264879,2.010101) -- (2.258636,1.969697) -- (2.252509,1.929293) -- (2.246511,1.888889) -- (2.240662,1.848485) -- (2.234986,1.808081) -- (2.229511,1.767677) -- (2.224266,1.727273) -- (2.219280,1.686869) -- (2.214578,1.646465) -- (2.210180,1.606061) -- (2.206096,1.565657) -- (2.202327,1.525253) -- (2.198859,1.484848) -- (2.195663,1.444444) -- (2.192697,1.404040) -- (2.189904,1.363636) -- (2.187215,1.323232) -- (2.184548,1.282828) -- (2.181816,1.242424) -- (2.178928,1.202020) -- (2.175793,1.161616) -- (2.172327,1.121212) -- (2.168454,1.080808) -- (2.164113,1.040404) -- (2.159257,1.000000) -- cycle;
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.032871,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.944749,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889834,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883967,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.075185,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.099061,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.025593,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055079,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.010470,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.104417,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.075805,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.880657,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.085777,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.888061,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055117,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.922157,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.087163,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009951,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951931,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981445,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.886797,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.909828,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.040950,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.035325,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027692,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.972083,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.119330,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115400,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.044530,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.036110,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.045227,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973341,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.912423,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.053157,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.006085,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.954458,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.996600,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093477,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.104170,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.965871,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.017167,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.957249,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.022632,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.961099,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973989,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093666,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.934518,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.029565,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.900164,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068904,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.937449,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.090356,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.894056,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.960668,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.916067,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.988081,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.071118,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.935354,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.892485,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.977092,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927643,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.901781,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.019280,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951687,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.041279,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927884,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.106107,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.967626,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.905319,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.030986,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102517,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.985691,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.109102,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.999975,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.982055,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.118823,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.107746,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.990411,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.999381,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.007035,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068589,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.979517,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.056276,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.050674,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.103694,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.907584,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.054964,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102582,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.112302,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883530,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.087274,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.109730,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.915703,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.113431,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093585,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.077370,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.995197,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.935770,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.072451,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.101647,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.943871,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009344,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.986261,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.103444,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889723,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055681,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027450,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.886808,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.052613,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883838,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.061908,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.003062,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102985,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.895860,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.081916,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.896006,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (2,2.000000) -- (2,4.000000);
\path[fill=white,draw=ink,line width=.45pt] (1.955,3.072225) -- (2,3.182225) -- (2.045,3.072225) -- (2,2.962225) -- cycle;


==> repo/figures/user_study/violin_cub_stats.tex <==
\draw[ink,line width=.45pt] (0,5.13) -- (0,5.20) -- (1,5.20) -- (1,5.13);
\node[anchor=south] at (0.5,5.20) {$^{**}$};
\draw[ink,line width=.45pt] (0,5.48) -- (0,5.55) -- (2,5.55) -- (2,5.48);
\node[anchor=south] at (1,5.55) {$^{***}$};


==> repo/figures/user_study/violin_data.tex <==
\path[fill=studyblue!35,draw=studyblue,line width=.45pt] (-0.070363,1.000000) -- (-0.070262,1.040404) -- (-0.069252,1.080808) -- (-0.067425,1.121212) -- (-0.064918,1.161616) -- (-0.061902,1.202020) -- (-0.058573,1.242424) -- (-0.055136,1.282828) -- (-0.051799,1.323232) -- (-0.048758,1.363636) -- (-0.046187,1.404040) -- (-0.044234,1.444444) -- (-0.043015,1.484848) -- (-0.042612,1.525253) -- (-0.043074,1.565657) -- (-0.044420,1.606061) -- (-0.046639,1.646465) -- (-0.049703,1.686869) -- (-0.053565,1.727273) -- (-0.058166,1.767677) -- (-0.063446,1.808081) -- (-0.069339,1.848485) -- (-0.075789,1.888889) -- (-0.082743,1.929293) -- (-0.090161,1.969697) -- (-0.098015,2.010101) -- (-0.106289,2.050505) -- (-0.114982,2.090909) -- (-0.124100,2.131313) -- (-0.133662,2.171717) -- (-0.143685,2.212121) -- (-0.154189,2.252525) -- (-0.165184,2.292929) -- (-0.176667,2.333333) -- (-0.188618,2.373737) -- (-0.200994,2.414141) -- (-0.213728,2.454545) -- (-0.226727,2.494949) -- (-0.239876,2.535354) -- (-0.253039,2.575758) -- (-0.266066,2.616162) -- (-0.278799,2.656566) -- (-0.291082,2.696970) -- (-0.302764,2.737374) -- (-0.313713,2.777778) -- (-0.323816,2.818182) -- (-0.332990,2.858586) -- (-0.341179,2.898990) -- (-0.348361,2.939394) -- (-0.354542,2.979798) -- (-0.359756,3.020202) -- (-0.364060,3.060606) -- (-0.367525,3.101010) -- (-0.370234,3.141414) -- (-0.372267,3.181818) -- (-0.373701,3.222222) -- (-0.374597,3.262626) -- (-0.375000,3.303030) -- (-0.374930,3.343434) -- (-0.374386,3.383838) -- (-0.373342,3.424242) -- (-0.371754,3.464646) -- (-0.369563,3.505051) -- (-0.366702,3.545455) -- (-0.363104,3.585859) -- (-0.358708,3.626263) -- (-0.353468,3.666667) -- (-0.347358,3.707071) -- (-0.340378,3.747475) -- (-0.332555,3.787879) -- (-0.323940,3.828283) -- (-0.314614,3.868687) -- (-0.304673,3.909091) -- (-0.294231,3.949495) -- (-0.283409,3.989899) -- (-0.272329,4.030303) -- (-0.261105,4.070707) -- (-0.249841,4.111111) -- (-0.238625,4.151515) -- (-0.227528,4.191919) -- (-0.216602,4.232323) -- (-0.205884,4.272727) -- (-0.195399,4.313131) -- (-0.185163,4.353535) -- (-0.175189,4.393939) -- (-0.165493,4.434343) -- (-0.156092,4.474747) -- (-0.147007,4.515152) -- (-0.138264,4.555556) -- (-0.129890,4.595960) -- (-0.121910,4.636364) -- (-0.114343,4.676768) -- (-0.107194,4.717172) -- (-0.100460,4.757576) -- (-0.094120,4.797980) -- (-0.088138,4.838384) -- (-0.082468,4.878788) -- (-0.077057,4.919192) -- (-0.071845,4.959596) -- (-0.066781,5.000000) -- (0.066781,5.000000) -- (0.071845,4.959596) -- (0.077057,4.919192) -- (0.082468,4.878788) -- (0.088138,4.838384) -- (0.094120,4.797980) -- (0.100460,4.757576) -- (0.107194,4.717172) -- (0.114343,4.676768) -- (0.121910,4.636364) -- (0.129890,4.595960) -- (0.138264,4.555556) -- (0.147007,4.515152) -- (0.156092,4.474747) -- (0.165493,4.434343) -- (0.175189,4.393939) -- (0.185163,4.353535) -- (0.195399,4.313131) -- (0.205884,4.272727) -- (0.216602,4.232323) -- (0.227528,4.191919) -- (0.238625,4.151515) -- (0.249841,4.111111) -- (0.261105,4.070707) -- (0.272329,4.030303) -- (0.283409,3.989899) -- (0.294231,3.949495) -- (0.304673,3.909091) -- (0.314614,3.868687) -- (0.323940,3.828283) -- (0.332555,3.787879) -- (0.340378,3.747475) -- (0.347358,3.707071) -- (0.353468,3.666667) -- (0.358708,3.626263) -- (0.363104,3.585859) -- (0.366702,3.545455) -- (0.369563,3.505051) -- (0.371754,3.464646) -- (0.373342,3.424242) -- (0.374386,3.383838) -- (0.374930,3.343434) -- (0.375000,3.303030) -- (0.374597,3.262626) -- (0.373701,3.222222) -- (0.372267,3.181818) -- (0.370234,3.141414) -- (0.367525,3.101010) -- (0.364060,3.060606) -- (0.359756,3.020202) -- (0.354542,2.979798) -- (0.348361,2.939394) -- (0.341179,2.898990) -- (0.332990,2.858586) -- (0.323816,2.818182) -- (0.313713,2.777778) -- (0.302764,2.737374) -- (0.291082,2.696970) -- (0.278799,2.656566) -- (0.266066,2.616162) -- (0.253039,2.575758) -- (0.239876,2.535354) -- (0.226727,2.494949) -- (0.213728,2.454545) -- (0.200994,2.414141) -- (0.188618,2.373737) -- (0.176667,2.333333) -- (0.165184,2.292929) -- (0.154189,2.252525) -- (0.143685,2.212121) -- (0.133662,2.171717) -- (0.124100,2.131313) -- (0.114982,2.090909) -- (0.106289,2.050505) -- (0.098015,2.010101) -- (0.090161,1.969697) -- (0.082743,1.929293) -- (0.075789,1.888889) -- (0.069339,1.848485) -- (0.063446,1.808081) -- (0.058166,1.767677) -- (0.053565,1.727273) -- (0.049703,1.686869) -- (0.046639,1.646465) -- (0.044420,1.606061) -- (0.043074,1.565657) -- (0.042612,1.525253) -- (0.043015,1.484848) -- (0.044234,1.444444) -- (0.046187,1.404040) -- (0.048758,1.363636) -- (0.051799,1.323232) -- (0.055136,1.282828) -- (0.058573,1.242424) -- (0.061902,1.202020) -- (0.064918,1.161616) -- (0.067425,1.121212) -- (0.069252,1.080808) -- (0.070262,1.040404) -- (0.070363,1.000000) -- cycle;
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.032871,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.055251,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110166,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116033,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.075185,4.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.099061,4.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.025593,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055079,1.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.010470,4.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.104417,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.075805,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.119343,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.085777,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.111939,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055117,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.077843,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.087163,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009951,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048069,4.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018555,2.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.113203,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.090172,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.040950,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.035325,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027692,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.027917,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.119330,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115400,3.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.044530,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.036110,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.045227,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026659,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.087577,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.053157,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.006085,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.045542,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.003400,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093477,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.104170,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.034129,4.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.017167,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.042751,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.022632,3.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.038901,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026011,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093666,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.065482,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.029565,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.099836,1.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068904,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.062551,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.090356,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.105944,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.039332,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.083933,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.011919,2.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.071118,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.064646,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.107515,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.022908,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072357,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.098219,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.019280,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048313,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.041279,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072116,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.106107,2.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.032374,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.094681,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.030986,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102517,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.014309,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.109102,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.000025,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.017945,2.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.118823,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.107746,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.009589,4.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.000619,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.007035,4.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068589,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.020483,2.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.056276,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.050674,3.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.103694,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.092416,2.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.054964,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102582,2.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.112302,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116470,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.087274,3.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.109730,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.084297,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.113431,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093585,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.077370,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.004803,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.064230,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.072451,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.101647,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.056129,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.009344,2.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.013739,3.285700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.103444,3.857100) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110277,3.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.055681,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027450,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.113192,3.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.052613,3.428600) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116162,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.061908,2.714300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.003062,2.142900) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102985,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.104140,2.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.081916,3.571400) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.103994,4.142900) circle[radius=.65pt];
\draw[ink,line width=2pt] (0,2.714300) -- (0,3.857100);
\path[fill=white,draw=ink,line width=.45pt] (-0.045,3.229761) -- (0,3.339761) -- (0.045,3.229761) -- (0,3.119761) -- cycle;
\path[fill=studypeach!35,draw=studypeach,line width=.45pt] (0.929170,1.000000) -- (0.929353,1.040404) -- (0.930461,1.080808) -- (0.932398,1.121212) -- (0.935022,1.161616) -- (0.938155,1.202020) -- (0.941597,1.242424) -- (0.945130,1.282828) -- (0.948542,1.323232) -- (0.951627,1.363636) -- (0.954203,1.404040) -- (0.956116,1.444444) -- (0.957244,1.484848) -- (0.957499,1.525253) -- (0.956828,1.565657) -- (0.955204,1.606061) -- (0.952625,1.646465) -- (0.949104,1.686869) -- (0.944666,1.727273) -- (0.939337,1.767677) -- (0.933140,1.808081) -- (0.926091,1.848485) -- (0.918197,1.888889) -- (0.909459,1.929293) -- (0.899869,1.969697) -- (0.889419,2.010101) -- (0.878106,2.050505) -- (0.865939,2.090909) -- (0.852945,2.131313) -- (0.839176,2.171717) -- (0.824714,2.212121) -- (0.809672,2.252525) -- (0.794197,2.292929) -- (0.778461,2.333333) -- (0.762662,2.373737) -- (0.747009,2.414141) -- (0.731718,2.454545) -- (0.716997,2.494949) -- (0.703041,2.535354) -- (0.690018,2.575758) -- (0.678064,2.616162) -- (0.667283,2.656566) -- (0.657740,2.696970) -- (0.649466,2.737374) -- (0.642462,2.777778) -- (0.636705,2.818182) -- (0.632154,2.858586) -- (0.628759,2.898990) -- (0.626466,2.939394) -- (0.625227,2.979798) -- (0.625000,3.020202) -- (0.625755,3.060606) -- (0.627474,3.101010) -- (0.630155,3.141414) -- (0.633804,3.181818) -- (0.638438,3.222222) -- (0.644079,3.262626) -- (0.650747,3.303030) -- (0.658460,3.343434) -- (0.667225,3.383838) -- (0.677031,3.424242) -- (0.687847,3.464646) -- (0.699616,3.505051) -- (0.712249,3.545455) -- (0.725627,3.585859) -- (0.739597,3.626263) -- (0.753978,3.666667) -- (0.768564,3.707071) -- (0.783132,3.747475) -- (0.797448,3.787879) -- (0.811282,3.828283) -- (0.824414,3.868687) -- (0.836648,3.909091) -- (0.847818,3.949495) -- (0.857798,3.989899) -- (0.866506,4.030303) -- (0.873906,4.070707) -- (0.880009,4.111111) -- (0.884868,4.151515) -- (0.888575,4.191919) -- (0.891255,4.232323) -- (0.893057,4.272727) -- (0.894147,4.313131) -- (0.894702,4.353535) -- (0.894899,4.393939) -- (0.894911,4.434343) -- (0.894903,4.474747) -- (0.895022,4.515152) -- (0.895398,4.555556) -- (0.896143,4.595960) -- (0.897341,4.636364) -- (0.899056,4.676768) -- (0.901326,4.717172) -- (0.904168,4.757576) -- (0.907574,4.797980) -- (0.911518,4.838384) -- (0.915953,4.878788) -- (0.920817,4.919192) -- (0.926035,4.959596) -- (0.931520,5.000000) -- (1.068480,5.000000) -- (1.073965,4.959596) -- (1.079183,4.919192) -- (1.084047,4.878788) -- (1.088482,4.838384) -- (1.092426,4.797980) -- (1.095832,4.757576) -- (1.098674,4.717172) -- (1.100944,4.676768) -- (1.102659,4.636364) -- (1.103857,4.595960) -- (1.104602,4.555556) -- (1.104978,4.515152) -- (1.105097,4.474747) -- (1.105089,4.434343) -- (1.105101,4.393939) -- (1.105298,4.353535) -- (1.105853,4.313131) -- (1.106943,4.272727) -- (1.108745,4.232323) -- (1.111425,4.191919) -- (1.115132,4.151515) -- (1.119991,4.111111) -- (1.126094,4.070707) -- (1.133494,4.030303) -- (1.142202,3.989899) -- (1.152182,3.949495) -- (1.163352,3.909091) -- (1.175586,3.868687) -- (1.188718,3.828283) -- (1.202552,3.787879) -- (1.216868,3.747475) -- (1.231436,3.707071) -- (1.246022,3.666667) -- (1.260403,3.626263) -- (1.274373,3.585859) -- (1.287751,3.545455) -- (1.300384,3.505051) -- (1.312153,3.464646) -- (1.322969,3.424242) -- (1.332775,3.383838) -- (1.341540,3.343434) -- (1.349253,3.303030) -- (1.355921,3.262626) -- (1.361562,3.222222) -- (1.366196,3.181818) -- (1.369845,3.141414) -- (1.372526,3.101010) -- (1.374245,3.060606) -- (1.375000,3.020202) -- (1.374773,2.979798) -- (1.373534,2.939394) -- (1.371241,2.898990) -- (1.367846,2.858586) -- (1.363295,2.818182) -- (1.357538,2.777778) -- (1.350534,2.737374) -- (1.342260,2.696970) -- (1.332717,2.656566) -- (1.321936,2.616162) -- (1.309982,2.575758) -- (1.296959,2.535354) -- (1.283003,2.494949) -- (1.268282,2.454545) -- (1.252991,2.414141) -- (1.237338,2.373737) -- (1.221539,2.333333) -- (1.205803,2.292929) -- (1.190328,2.252525) -- (1.175286,2.212121) -- (1.160824,2.171717) -- (1.147055,2.131313) -- (1.134061,2.090909) -- (1.121894,2.050505) -- (1.110581,2.010101) -- (1.100131,1.969697) -- (1.090541,1.929293) -- (1.081803,1.888889) -- (1.073909,1.848485) -- (1.066860,1.808081) -- (1.060663,1.767677) -- (1.055334,1.727273) -- (1.050896,1.686869) -- (1.047375,1.646465) -- (1.044796,1.606061) -- (1.043172,1.565657) -- (1.042501,1.525253) -- (1.042756,1.484848) -- (1.043884,1.444444) -- (1.045797,1.404040) -- (1.048373,1.363636) -- (1.051458,1.323232) -- (1.054870,1.282828) -- (1.058403,1.242424) -- (1.061845,1.202020) -- (1.064978,1.161616) -- (1.067602,1.121212) -- (1.069539,1.080808) -- (1.070647,1.040404) -- (1.070830,1.000000) -- cycle;
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.032871,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.944749,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889834,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883967,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.075185,4.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.099061,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.025593,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055079,1.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.010470,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.104417,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.075805,2.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.880657,4.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.085777,2.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.888061,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055117,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.922157,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.087163,4.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009951,4.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951931,4.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981445,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.886797,2.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.909828,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.040950,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.035325,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027692,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.972083,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.119330,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115400,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.044530,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.036110,4.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.045227,4.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973341,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.912423,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.053157,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.006085,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.954458,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.996600,4.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093477,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.104170,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.965871,4.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.017167,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.957249,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.022632,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.961099,3.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973989,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093666,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.934518,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.029565,1.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.900164,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068904,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.937449,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.090356,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.894056,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.960668,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.916067,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.988081,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.071118,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.935354,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.892485,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.977092,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927643,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.901781,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.019280,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951687,4.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.041279,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927884,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.106107,1.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.967626,4.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.905319,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.030986,4.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102517,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.985691,2.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.109102,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.999975,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.982055,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.118823,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.107746,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.990411,3.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.999381,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.007035,4.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068589,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.979517,2.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.056276,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.050674,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.103694,4.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.907584,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.054964,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102582,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.112302,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883530,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.087274,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.109730,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.915703,2.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.113431,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093585,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.077370,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.995197,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.935770,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.072451,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.101647,2.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.943871,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.009344,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.986261,2.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.103444,3.285700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889723,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.055681,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027450,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.886808,3.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.052613,3.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883838,2.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.061908,2.714300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.003062,2.142900) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102985,3.571400) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.895860,2.857100) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.081916,2.428600) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.896006,4.142900) circle[radius=.65pt];
\draw[ink,line width=2pt] (1,2.571400) -- (1,3.571400);
\path[fill=white,draw=ink,line width=.45pt] (0.955,3.066663) -- (1,3.176663) -- (1.045,3.066663) -- (1,2.956663) -- cycle;
\path[fill=studygray!35,draw=studygray,line width=.45pt] (1.913426,1.000000) -- (1.911043,1.040404) -- (1.909514,1.080808) -- (1.908800,1.121212) -- (1.908821,1.161616) -- (1.909457,1.202020) -- (1.910559,1.242424) -- (1.911960,1.282828) -- (1.913478,1.323232) -- (1.914933,1.363636) -- (1.916150,1.404040) -- (1.916968,1.444444) -- (1.917249,1.484848) -- (1.916875,1.525253) -- (1.915752,1.565657) -- (1.913813,1.606061) -- (1.911012,1.646465) -- (1.907321,1.686869) -- (1.902733,1.727273) -- (1.897254,1.767677) -- (1.890900,1.808081) -- (1.883697,1.848485) -- (1.875681,1.888889) -- (1.866888,1.929293) -- (1.857364,1.969697) -- (1.847153,2.010101) -- (1.836305,2.050505) -- (1.824871,2.090909) -- (1.812903,2.131313) -- (1.800459,2.171717) -- (1.787600,2.212121) -- (1.774393,2.252525) -- (1.760916,2.292929) -- (1.747259,2.333333) -- (1.733528,2.373737) -- (1.719849,2.414141) -- (1.706366,2.454545) -- (1.693250,2.494949) -- (1.680687,2.535354) -- (1.668885,2.575758) -- (1.658060,2.616162) -- (1.648435,2.656566) -- (1.640223,2.696970) -- (1.633624,2.737374) -- (1.628807,2.777778) -- (1.625904,2.818182) -- (1.625000,2.858586) -- (1.626125,2.898990) -- (1.629252,2.939394) -- (1.634298,2.979798) -- (1.641127,3.020202) -- (1.649555,3.060606) -- (1.659364,3.101010) -- (1.670306,3.141414) -- (1.682123,3.181818) -- (1.694553,3.222222) -- (1.707344,3.262626) -- (1.720261,3.303030) -- (1.733098,3.343434) -- (1.745677,3.383838) -- (1.757854,3.424242) -- (1.769518,3.464646) -- (1.780592,3.505051) -- (1.791026,3.545455) -- (1.800798,3.585859) -- (1.809905,3.626263) -- (1.818366,3.666667) -- (1.826210,3.707071) -- (1.833480,3.747475) -- (1.840228,3.787879) -- (1.846509,3.828283) -- (1.852384,3.868687) -- (1.857914,3.909091) -- (1.863158,3.949495) -- (1.868172,3.989899) -- (1.873003,4.030303) -- (1.877693,4.070707) -- (1.882270,4.111111) -- (1.886753,4.151515) -- (1.891145,4.191919) -- (1.895444,4.232323) -- (1.899633,4.272727) -- (1.903694,4.313131) -- (1.907603,4.353535) -- (1.911339,4.393939) -- (1.914886,4.434343) -- (1.918235,4.474747) -- (1.921389,4.515152) -- (1.924360,4.555556) -- (1.927175,4.595960) -- (1.929868,4.636364) -- (1.932482,4.676768) -- (1.935066,4.717172) -- (1.937667,4.757576) -- (1.940331,4.797980) -- (1.943095,4.838384) -- (1.945989,4.878788) -- (1.949027,4.919192) -- (1.952212,4.959596) -- (1.955531,5.000000) -- (2.044469,5.000000) -- (2.047788,4.959596) -- (2.050973,4.919192) -- (2.054011,4.878788) -- (2.056905,4.838384) -- (2.059669,4.797980) -- (2.062333,4.757576) -- (2.064934,4.717172) -- (2.067518,4.676768) -- (2.070132,4.636364) -- (2.072825,4.595960) -- (2.075640,4.555556) -- (2.078611,4.515152) -- (2.081765,4.474747) -- (2.085114,4.434343) -- (2.088661,4.393939) -- (2.092397,4.353535) -- (2.096306,4.313131) -- (2.100367,4.272727) -- (2.104556,4.232323) -- (2.108855,4.191919) -- (2.113247,4.151515) -- (2.117730,4.111111) -- (2.122307,4.070707) -- (2.126997,4.030303) -- (2.131828,3.989899) -- (2.136842,3.949495) -- (2.142086,3.909091) -- (2.147616,3.868687) -- (2.153491,3.828283) -- (2.159772,3.787879) -- (2.166520,3.747475) -- (2.173790,3.707071) -- (2.181634,3.666667) -- (2.190095,3.626263) -- (2.199202,3.585859) -- (2.208974,3.545455) -- (2.219408,3.505051) -- (2.230482,3.464646) -- (2.242146,3.424242) -- (2.254323,3.383838) -- (2.266902,3.343434) -- (2.279739,3.303030) -- (2.292656,3.262626) -- (2.305447,3.222222) -- (2.317877,3.181818) -- (2.329694,3.141414) -- (2.340636,3.101010) -- (2.350445,3.060606) -- (2.358873,3.020202) -- (2.365702,2.979798) -- (2.370748,2.939394) -- (2.373875,2.898990) -- (2.375000,2.858586) -- (2.374096,2.818182) -- (2.371193,2.777778) -- (2.366376,2.737374) -- (2.359777,2.696970) -- (2.351565,2.656566) -- (2.341940,2.616162) -- (2.331115,2.575758) -- (2.319313,2.535354) -- (2.306750,2.494949) -- (2.293634,2.454545) -- (2.280151,2.414141) -- (2.266472,2.373737) -- (2.252741,2.333333) -- (2.239084,2.292929) -- (2.225607,2.252525) -- (2.212400,2.212121) -- (2.199541,2.171717) -- (2.187097,2.131313) -- (2.175129,2.090909) -- (2.163695,2.050505) -- (2.152847,2.010101) -- (2.142636,1.969697) -- (2.133112,1.929293) -- (2.124319,1.888889) -- (2.116303,1.848485) -- (2.109100,1.808081) -- (2.102746,1.767677) -- (2.097267,1.727273) -- (2.092679,1.686869) -- (2.088988,1.646465) -- (2.086187,1.606061) -- (2.084248,1.565657) -- (2.083125,1.525253) -- (2.082751,1.484848) -- (2.083032,1.444444) -- (2.083850,1.404040) -- (2.085067,1.363636) -- (2.086522,1.323232) -- (2.088040,1.282828) -- (2.089441,1.242424) -- (2.090543,1.202020) -- (2.091179,1.161616) -- (2.091200,1.121212) -- (2.090486,1.080808) -- (2.088957,1.040404) -- (2.086574,1.000000) -- cycle;
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.032871,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.944749,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889834,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883967,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.075185,4.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.099061,3.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.025593,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055079,1.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.010470,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.104417,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.075805,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.880657,2.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.085777,1.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.888061,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055117,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.922157,3.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.087163,4.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009951,4.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951931,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981445,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.886797,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.909828,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.040950,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.035325,2.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027692,2.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.972083,2.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.119330,3.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115400,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.044530,3.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.036110,3.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.045227,4.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973341,2.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.912423,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.053157,1.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.006085,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.954458,3.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.996600,3.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093477,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.104170,4.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.965871,4.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.017167,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.957249,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.022632,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.961099,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973989,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093666,1.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.934518,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.029565,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.900164,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.079835,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068904,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.937449,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.090356,2.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.894056,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.960668,3.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.916067,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.988081,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.071118,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.935354,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.892485,1.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.977092,1.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927643,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.901781,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.019280,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951687,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.041279,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927884,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.106107,1.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.967626,4.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.905319,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.030986,4.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102517,2.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.985691,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.109102,1.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.999975,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.982055,2.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.028851,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.118823,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.107746,2.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.990411,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.061855,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.999381,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.007035,3.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068589,3.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.979517,1.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.056276,3.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.050674,3.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.103694,4.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.907584,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.054964,4.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102582,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.112302,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883530,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.087274,3.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115487,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.109730,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.915703,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.113431,3.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093585,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.077370,3.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.995197,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.935770,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.072451,3.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.101647,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.943871,3.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.009344,2.714300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.986261,3.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.103444,3.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889723,2.428600) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.055681,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027450,2.285700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.886808,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.052613,4.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883838,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.061908,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.003062,2.571400) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102985,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.895860,3.142900) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.081916,2.857100) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.896006,4.142900) circle[radius=.65pt];
\draw[ink,line width=2pt] (2,2.428600) -- (2,3.428600);
\path[fill=white,draw=ink,line width=.45pt] (1.955,2.873811) -- (2,2.983811) -- (2.045,2.873811) -- (2,2.763811) -- cycle;


==> repo/figures/user_study/violin_partimagenet_data.tex <==
\path[fill=studyblue!35,draw=studyblue,line width=.45pt] (-0.170560,1.000000) -- (-0.174420,1.040404) -- (-0.177304,1.080808) -- (-0.179299,1.121212) -- (-0.180532,1.161616) -- (-0.181158,1.202020) -- (-0.181356,1.242424) -- (-0.181320,1.282828) -- (-0.181246,1.323232) -- (-0.181326,1.363636) -- (-0.181733,1.404040) -- (-0.182619,1.444444) -- (-0.184106,1.484848) -- (-0.186279,1.525253) -- (-0.189190,1.565657) -- (-0.192852,1.606061) -- (-0.197243,1.646465) -- (-0.202313,1.686869) -- (-0.207985,1.727273) -- (-0.214161,1.767677) -- (-0.220735,1.808081) -- (-0.227594,1.848485) -- (-0.234627,1.888889) -- (-0.241733,1.929293) -- (-0.248822,1.969697) -- (-0.255823,2.010101) -- (-0.262686,2.050505) -- (-0.269380,2.090909) -- (-0.275894,2.131313) -- (-0.282238,2.171717) -- (-0.288434,2.212121) -- (-0.294515,2.252525) -- (-0.300521,2.292929) -- (-0.306489,2.333333) -- (-0.312452,2.373737) -- (-0.318432,2.414141) -- (-0.324435,2.454545) -- (-0.330447,2.494949) -- (-0.336434,2.535354) -- (-0.342338,2.575758) -- (-0.348083,2.616162) -- (-0.353570,2.656566) -- (-0.358687,2.696970) -- (-0.363313,2.737374) -- (-0.367323,2.777778) -- (-0.370597,2.818182) -- (-0.373024,2.858586) -- (-0.374514,2.898990) -- (-0.375000,2.939394) -- (-0.374446,2.979798) -- (-0.372851,3.020202) -- (-0.370247,3.060606) -- (-0.366703,3.101010) -- (-0.362322,3.141414) -- (-0.357235,3.181818) -- (-0.351593,3.222222) -- (-0.345564,3.262626) -- (-0.339321,3.303030) -- (-0.333032,3.343434) -- (-0.326852,3.383838) -- (-0.320912,3.424242) -- (-0.315315,3.464646) -- (-0.310124,3.505051) -- (-0.305366,3.545455) -- (-0.301024,3.585859) -- (-0.297043,3.626263) -- (-0.293331,3.666667) -- (-0.289766,3.707071) -- (-0.286205,3.747475) -- (-0.282496,3.787879) -- (-0.278482,3.828283) -- (-0.274021,3.868687) -- (-0.268989,3.909091) -- (-0.263292,3.949495) -- (-0.256872,3.989899) -- (-0.249712,4.030303) -- (-0.241838,4.070707) -- (-0.233318,4.111111) -- (-0.224257,4.151515) -- (-0.214792,4.191919) -- (-0.205082,4.232323) -- (-0.195300,4.272727) -- (-0.185622,4.313131) -- (-0.176217,4.353535) -- (-0.167235,4.393939) -- (-0.158804,4.434343) -- (-0.151019,4.474747) -- (-0.143938,4.515152) -- (-0.137583,4.555556) -- (-0.131941,4.595960) -- (-0.126961,4.636364) -- (-0.122565,4.676768) -- (-0.118653,4.717172) -- (-0.115106,4.757576) -- (-0.111799,4.797980) -- (-0.108606,4.838384) -- (-0.105409,4.878788) -- (-0.102101,4.919192) -- (-0.098594,4.959596) -- (-0.094824,5.000000) -- (0.094824,5.000000) -- (0.098594,4.959596) -- (0.102101,4.919192) -- (0.105409,4.878788) -- (0.108606,4.838384) -- (0.111799,4.797980) -- (0.115106,4.757576) -- (0.118653,4.717172) -- (0.122565,4.676768) -- (0.126961,4.636364) -- (0.131941,4.595960) -- (0.137583,4.555556) -- (0.143938,4.515152) -- (0.151019,4.474747) -- (0.158804,4.434343) -- (0.167235,4.393939) -- (0.176217,4.353535) -- (0.185622,4.313131) -- (0.195300,4.272727) -- (0.205082,4.232323) -- (0.214792,4.191919) -- (0.224257,4.151515) -- (0.233318,4.111111) -- (0.241838,4.070707) -- (0.249712,4.030303) -- (0.256872,3.989899) -- (0.263292,3.949495) -- (0.268989,3.909091) -- (0.274021,3.868687) -- (0.278482,3.828283) -- (0.282496,3.787879) -- (0.286205,3.747475) -- (0.289766,3.707071) -- (0.293331,3.666667) -- (0.297043,3.626263) -- (0.301024,3.585859) -- (0.305366,3.545455) -- (0.310124,3.505051) -- (0.315315,3.464646) -- (0.320912,3.424242) -- (0.326852,3.383838) -- (0.333032,3.343434) -- (0.339321,3.303030) -- (0.345564,3.262626) -- (0.351593,3.222222) -- (0.357235,3.181818) -- (0.362322,3.141414) -- (0.366703,3.101010) -- (0.370247,3.060606) -- (0.372851,3.020202) -- (0.374446,2.979798) -- (0.375000,2.939394) -- (0.374514,2.898990) -- (0.373024,2.858586) -- (0.370597,2.818182) -- (0.367323,2.777778) -- (0.363313,2.737374) -- (0.358687,2.696970) -- (0.353570,2.656566) -- (0.348083,2.616162) -- (0.342338,2.575758) -- (0.336434,2.535354) -- (0.330447,2.494949) -- (0.324435,2.454545) -- (0.318432,2.414141) -- (0.312452,2.373737) -- (0.306489,2.333333) -- (0.300521,2.292929) -- (0.294515,2.252525) -- (0.288434,2.212121) -- (0.282238,2.171717) -- (0.275894,2.131313) -- (0.269380,2.090909) -- (0.262686,2.050505) -- (0.255823,2.010101) -- (0.248822,1.969697) -- (0.241733,1.929293) -- (0.234627,1.888889) -- (0.227594,1.848485) -- (0.220735,1.808081) -- (0.214161,1.767677) -- (0.207985,1.727273) -- (0.202313,1.686869) -- (0.197243,1.646465) -- (0.192852,1.606061) -- (0.189190,1.565657) -- (0.186279,1.525253) -- (0.184106,1.484848) -- (0.182619,1.444444) -- (0.181733,1.404040) -- (0.181326,1.363636) -- (0.181246,1.323232) -- (0.181320,1.282828) -- (0.181356,1.242424) -- (0.181158,1.202020) -- (0.180532,1.161616) -- (0.179299,1.121212) -- (0.177304,1.080808) -- (0.174420,1.040404) -- (0.170560,1.000000) -- cycle;
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.057213,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048362,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.075414,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.097940,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.024024,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.054855,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.074904,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.106765,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.054007,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.037784,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.014944,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.083985,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.016169,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.040631,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.018532,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.031964,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.112185,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.043936,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026010,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.075059,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.036969,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.002656,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.093890,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.066135,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.043645,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.101812,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.006982,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.046502,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.094270,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.094910,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.071542,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.092268,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.043155,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.083817,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.034665,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.022430,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.003979,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.022426,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.086908,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.014835,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.094138,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027292,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.079045,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.000467,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.046204,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.038634,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.005479,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.068106,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.095831,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.110735,5.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.048468,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.010457,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.095456,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.080444,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.027577,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.113683,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.022095,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.063812,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.022273,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.072919,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.078774,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.076511,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.024913,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.092968,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.115221,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.079919,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.096141,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.011860,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.002760,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.028865,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.000963,4.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.104962,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.060095,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.017872,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.028145,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.001572,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.111543,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.065610,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.045367,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.013223,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.109917,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048924,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.102520,4.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.068296,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.116921,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.048810,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.117647,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.078592,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.093512,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.106211,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.115652,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.012991,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.043586,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.108237,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.026497,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.032151,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.005635,2.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.118371,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.084489,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.069627,4.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.014279,1.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.047447,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027199,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.051496,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.098312,2.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.110849,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.105736,3.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.069826,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.015126,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.064958,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.104634,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.075647,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.010387,2.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.040486,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.096799,1.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.088074,1.333300) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.070501,3.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (-0.107344,1.666700) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.114393,3.000000) circle[radius=.65pt];
\filldraw[fill=studyblue!70!black,draw=white,line width=.15pt] (0.027511,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (0,2.000000) -- (0,3.666700);
\path[fill=white,draw=ink,line width=.45pt] (-0.045,2.861112) -- (0,2.971112) -- (0.045,2.861112) -- (0,2.751112) -- cycle;
\path[fill=studypeach!35,draw=studypeach,line width=.45pt] (0.869717,1.000000) -- (0.865621,1.040404) -- (0.862095,1.080808) -- (0.858987,1.121212) -- (0.856100,1.161616) -- (0.853202,1.202020) -- (0.850035,1.242424) -- (0.846335,1.282828) -- (0.841845,1.323232) -- (0.836329,1.363636) -- (0.829593,1.404040) -- (0.821496,1.444444) -- (0.811960,1.484848) -- (0.800981,1.525253) -- (0.788632,1.565657) -- (0.775063,1.606061) -- (0.760495,1.646465) -- (0.745214,1.686869) -- (0.729553,1.727273) -- (0.713882,1.767677) -- (0.698586,1.808081) -- (0.684043,1.848485) -- (0.670609,1.888889) -- (0.658595,1.929293) -- (0.648252,1.969697) -- (0.639760,2.010101) -- (0.633216,2.050505) -- (0.628633,2.090909) -- (0.625943,2.131313) -- (0.625000,2.171717) -- (0.625592,2.212121) -- (0.627460,2.252525) -- (0.630309,2.292929) -- (0.633832,2.333333) -- (0.637730,2.373737) -- (0.641724,2.414141) -- (0.645581,2.454545) -- (0.649117,2.494949) -- (0.652215,2.535354) -- (0.654824,2.575758) -- (0.656965,2.616162) -- (0.658720,2.656566) -- (0.660230,2.696970) -- (0.661680,2.737374) -- (0.663281,2.777778) -- (0.665260,2.818182) -- (0.667838,2.858586) -- (0.671211,2.898990) -- (0.675541,2.939394) -- (0.680936,2.979798) -- (0.687448,3.020202) -- (0.695064,3.060606) -- (0.703707,3.101010) -- (0.713240,3.141414) -- (0.723478,3.181818) -- (0.734194,3.222222) -- (0.745140,3.262626) -- (0.756055,3.303030) -- (0.766689,3.343434) -- (0.776811,3.383838) -- (0.786229,3.424242) -- (0.794793,3.464646) -- (0.802406,3.505051) -- (0.809028,3.545455) -- (0.814675,3.585859) -- (0.819414,3.626263) -- (0.823360,3.666667) -- (0.826662,3.707071) -- (0.829498,3.747475) -- (0.832056,3.787879) -- (0.834530,3.828283) -- (0.837099,3.868687) -- (0.839925,3.909091) -- (0.843137,3.949495) -- (0.846829,3.989899) -- (0.851052,4.030303) -- (0.855815,4.070707) -- (0.861085,4.111111) -- (0.866792,4.151515) -- (0.872833,4.191919) -- (0.879081,4.232323) -- (0.885393,4.272727) -- (0.891621,4.313131) -- (0.897621,4.353535) -- (0.903259,4.393939) -- (0.908425,4.434343) -- (0.913034,4.474747) -- (0.917032,4.515152) -- (0.920399,4.555556) -- (0.923149,4.595960) -- (0.925329,4.636364) -- (0.927012,4.676768) -- (0.928298,4.717172) -- (0.929300,4.757576) -- (0.930142,4.797980) -- (0.930952,4.838384) -- (0.931849,4.878788) -- (0.932941,4.919192) -- (0.934319,4.959596) -- (0.936048,5.000000) -- (1.063952,5.000000) -- (1.065681,4.959596) -- (1.067059,4.919192) -- (1.068151,4.878788) -- (1.069048,4.838384) -- (1.069858,4.797980) -- (1.070700,4.757576) -- (1.071702,4.717172) -- (1.072988,4.676768) -- (1.074671,4.636364) -- (1.076851,4.595960) -- (1.079601,4.555556) -- (1.082968,4.515152) -- (1.086966,4.474747) -- (1.091575,4.434343) -- (1.096741,4.393939) -- (1.102379,4.353535) -- (1.108379,4.313131) -- (1.114607,4.272727) -- (1.120919,4.232323) -- (1.127167,4.191919) -- (1.133208,4.151515) -- (1.138915,4.111111) -- (1.144185,4.070707) -- (1.148948,4.030303) -- (1.153171,3.989899) -- (1.156863,3.949495) -- (1.160075,3.909091) -- (1.162901,3.868687) -- (1.165470,3.828283) -- (1.167944,3.787879) -- (1.170502,3.747475) -- (1.173338,3.707071) -- (1.176640,3.666667) -- (1.180586,3.626263) -- (1.185325,3.585859) -- (1.190972,3.545455) -- (1.197594,3.505051) -- (1.205207,3.464646) -- (1.213771,3.424242) -- (1.223189,3.383838) -- (1.233311,3.343434) -- (1.243945,3.303030) -- (1.254860,3.262626) -- (1.265806,3.222222) -- (1.276522,3.181818) -- (1.286760,3.141414) -- (1.296293,3.101010) -- (1.304936,3.060606) -- (1.312552,3.020202) -- (1.319064,2.979798) -- (1.324459,2.939394) -- (1.328789,2.898990) -- (1.332162,2.858586) -- (1.334740,2.818182) -- (1.336719,2.777778) -- (1.338320,2.737374) -- (1.339770,2.696970) -- (1.341280,2.656566) -- (1.343035,2.616162) -- (1.345176,2.575758) -- (1.347785,2.535354) -- (1.350883,2.494949) -- (1.354419,2.454545) -- (1.358276,2.414141) -- (1.362270,2.373737) -- (1.366168,2.333333) -- (1.369691,2.292929) -- (1.372540,2.252525) -- (1.374408,2.212121) -- (1.375000,2.171717) -- (1.374057,2.131313) -- (1.371367,2.090909) -- (1.366784,2.050505) -- (1.360240,2.010101) -- (1.351748,1.969697) -- (1.341405,1.929293) -- (1.329391,1.888889) -- (1.315957,1.848485) -- (1.301414,1.808081) -- (1.286118,1.767677) -- (1.270447,1.727273) -- (1.254786,1.686869) -- (1.239505,1.646465) -- (1.224937,1.606061) -- (1.211368,1.565657) -- (1.199019,1.525253) -- (1.188040,1.484848) -- (1.178504,1.444444) -- (1.170407,1.404040) -- (1.163671,1.363636) -- (1.158155,1.323232) -- (1.153665,1.282828) -- (1.149965,1.242424) -- (1.146798,1.202020) -- (1.143900,1.161616) -- (1.141013,1.121212) -- (1.137905,1.080808) -- (1.134379,1.040404) -- (1.130283,1.000000) -- cycle;
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.942787,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951638,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.075414,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.902060,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.024024,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.054855,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.925096,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.893235,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.945993,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.037784,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.014944,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.916015,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.983831,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.040631,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.981468,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.031964,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.112185,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.043936,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973990,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.924941,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.963031,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.002656,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.093890,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.066135,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.956355,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.101812,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.993018,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.046502,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.905730,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.905090,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.928458,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.092268,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.043155,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.083817,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.034665,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.977570,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.003979,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.022426,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.086908,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.985165,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.094138,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027292,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.079045,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.999533,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.046204,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.961366,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.005479,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.931894,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.904169,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.889265,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.048468,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.989543,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.095456,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.080444,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.972423,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.113683,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.022095,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.063812,4.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.977727,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.927081,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.921226,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.923489,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.024913,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.907032,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.884779,5.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.079919,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.903859,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.988140,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.997240,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.028865,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.000963,4.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.104962,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.060095,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.017872,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.028145,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.001572,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.111543,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.934390,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.045367,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.013223,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.890083,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951076,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.102520,4.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.068296,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.883079,1.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.951190,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.882353,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.078592,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.906488,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.893789,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.115652,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.987009,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.956414,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.891763,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.973503,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.967849,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.005635,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.881629,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.915511,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.930373,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.985721,1.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.952553,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027199,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.948504,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.098312,3.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.110849,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.894264,1.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.930174,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.015126,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.064958,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.895366,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.924353,2.666700) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.989613,3.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.040486,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.096799,1.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.088074,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.070501,2.000000) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (0.892656,3.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.114393,2.333300) circle[radius=.65pt];
\filldraw[fill=studypeach!70!black,draw=white,line width=.15pt] (1.027511,4.000000) circle[radius=.65pt];
\draw[ink,line width=2pt] (1,2.000000) -- (1,3.083325);
\path[fill=white,draw=ink,line width=.45pt] (0.955,2.669444) -- (1,2.779444) -- (1.045,2.669444) -- (1,2.559444) -- cycle;
\path[fill=studygray!35,draw=studygray,line width=.45pt] (1.784788,1.000000) -- (1.778105,1.040404) -- (1.772612,1.080808) -- (1.768227,1.121212) -- (1.764815,1.161616) -- (1.762201,1.202020) -- (1.760175,1.242424) -- (1.758510,1.282828) -- (1.756971,1.323232) -- (1.755334,1.363636) -- (1.753396,1.404040) -- (1.750987,1.444444) -- (1.747982,1.484848) -- (1.744307,1.525253) -- (1.739941,1.565657) -- (1.734919,1.606061) -- (1.729324,1.646465) -- (1.723286,1.686869) -- (1.716970,1.727273) -- (1.710561,1.767677) -- (1.704257,1.808081) -- (1.698252,1.848485) -- (1.692724,1.888889) -- (1.687820,1.929293) -- (1.683650,1.969697) -- (1.680275,2.010101) -- (1.677707,2.050505) -- (1.675904,2.090909) -- (1.674773,2.131313) -- (1.674181,2.171717) -- (1.673955,2.212121) -- (1.673902,2.252525) -- (1.673817,2.292929) -- (1.673499,2.333333) -- (1.672765,2.373737) -- (1.671464,2.414141) -- (1.669487,2.454545) -- (1.666779,2.494949) -- (1.663342,2.535354) -- (1.659238,2.575758) -- (1.654590,2.616162) -- (1.649574,2.656566) -- (1.644412,2.696970) -- (1.639358,2.737374) -- (1.634684,2.777778) -- (1.630667,2.818182) -- (1.627567,2.858586) -- (1.625616,2.898990) -- (1.625000,2.939394) -- (1.625847,2.979798) -- (1.628221,3.020202) -- (1.632113,3.060606) -- (1.637444,3.101010) -- (1.644066,3.141414) -- (1.651773,3.181818) -- (1.660310,3.222222) -- (1.669387,3.262626) -- (1.678701,3.303030) -- (1.687944,3.343434) -- (1.696829,3.383838) -- (1.705103,3.424242) -- (1.712559,3.464646) -- (1.719051,3.505051) -- (1.724496,3.545455) -- (1.728883,3.585859) -- (1.732266,3.626263) -- (1.734767,3.666667) -- (1.736558,3.707071) -- (1.737856,3.747475) -- (1.738906,3.787879) -- (1.739967,3.828283) -- (1.741296,3.868687) -- (1.743130,3.909091) -- (1.745678,3.949495) -- (1.749105,3.989899) -- (1.753528,4.030303) -- (1.759007,4.070707) -- (1.765550,4.111111) -- (1.773110,4.151515) -- (1.781594,4.191919) -- (1.790871,4.232323) -- (1.800781,4.272727) -- (1.811146,4.313131) -- (1.821784,4.353535) -- (1.832514,4.393939) -- (1.843168,4.434343) -- (1.853601,4.474747) -- (1.863691,4.515152) -- (1.873345,4.555556) -- (1.882498,4.595960) -- (1.891112,4.636364) -- (1.899178,4.676768) -- (1.906702,4.717172) -- (1.913712,4.757576) -- (1.920244,4.797980) -- (1.926341,4.838384) -- (1.932051,4.878788) -- (1.937416,4.919192) -- (1.942479,4.959596) -- (1.947274,5.000000) -- (2.052726,5.000000) -- (2.057521,4.959596) -- (2.062584,4.919192) -- (2.067949,4.878788) -- (2.073659,4.838384) -- (2.079756,4.797980) -- (2.086288,4.757576) -- (2.093298,4.717172) -- (2.100822,4.676768) -- (2.108888,4.636364) -- (2.117502,4.595960) -- (2.126655,4.555556) -- (2.136309,4.515152) -- (2.146399,4.474747) -- (2.156832,4.434343) -- (2.167486,4.393939) -- (2.178216,4.353535) -- (2.188854,4.313131) -- (2.199219,4.272727) -- (2.209129,4.232323) -- (2.218406,4.191919) -- (2.226890,4.151515) -- (2.234450,4.111111) -- (2.240993,4.070707) -- (2.246472,4.030303) -- (2.250895,3.989899) -- (2.254322,3.949495) -- (2.256870,3.909091) -- (2.258704,3.868687) -- (2.260033,3.828283) -- (2.261094,3.787879) -- (2.262144,3.747475) -- (2.263442,3.707071) -- (2.265233,3.666667) -- (2.267734,3.626263) -- (2.271117,3.585859) -- (2.275504,3.545455) -- (2.280949,3.505051) -- (2.287441,3.464646) -- (2.294897,3.424242) -- (2.303171,3.383838) -- (2.312056,3.343434) -- (2.321299,3.303030) -- (2.330613,3.262626) -- (2.339690,3.222222) -- (2.348227,3.181818) -- (2.355934,3.141414) -- (2.362556,3.101010) -- (2.367887,3.060606) -- (2.371779,3.020202) -- (2.374153,2.979798) -- (2.375000,2.939394) -- (2.374384,2.898990) -- (2.372433,2.858586) -- (2.369333,2.818182) -- (2.365316,2.777778) -- (2.360642,2.737374) -- (2.355588,2.696970) -- (2.350426,2.656566) -- (2.345410,2.616162) -- (2.340762,2.575758) -- (2.336658,2.535354) -- (2.333221,2.494949) -- (2.330513,2.454545) -- (2.328536,2.414141) -- (2.327235,2.373737) -- (2.326501,2.333333) -- (2.326183,2.292929) -- (2.326098,2.252525) -- (2.326045,2.212121) -- (2.325819,2.171717) -- (2.325227,2.131313) -- (2.324096,2.090909) -- (2.322293,2.050505) -- (2.319725,2.010101) -- (2.316350,1.969697) -- (2.312180,1.929293) -- (2.307276,1.888889) -- (2.301748,1.848485) -- (2.295743,1.808081) -- (2.289439,1.767677) -- (2.283030,1.727273) -- (2.276714,1.686869) -- (2.270676,1.646465) -- (2.265081,1.606061) -- (2.260059,1.565657) -- (2.255693,1.525253) -- (2.252018,1.484848) -- (2.249013,1.444444) -- (2.246604,1.404040) -- (2.244666,1.363636) -- (2.243029,1.323232) -- (2.241490,1.282828) -- (2.239825,1.242424) -- (2.237799,1.202020) -- (2.235185,1.161616) -- (2.231773,1.121212) -- (2.227388,1.080808) -- (2.221895,1.040404) -- (2.215212,1.000000) -- cycle;
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.942787,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951638,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.075414,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.902060,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.024024,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.054855,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.925096,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.893235,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.945993,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.037784,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.014944,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.916015,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.983831,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.040631,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.981468,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.031964,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.112185,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.043936,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973990,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.924941,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.963031,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.002656,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.093890,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.066135,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.956355,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.101812,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.993018,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.046502,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.905730,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.905090,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.928458,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.092268,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.043155,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.083817,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.034665,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.977570,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.003979,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.022426,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.086908,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.985165,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.094138,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027292,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.079045,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.999533,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.046204,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.961366,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.005479,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.931894,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.904169,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.889265,5.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.048468,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.989543,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.095456,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.080444,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.972423,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.113683,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.022095,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.063812,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.977727,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.927081,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.921226,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.923489,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.024913,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.907032,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.884779,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.079919,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.903859,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.988140,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.997240,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.028865,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.000963,4.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.104962,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.060095,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.017872,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.028145,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.001572,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.111543,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.934390,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.045367,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.013223,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.890083,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951076,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.102520,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.068296,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.883079,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.951190,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.882353,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.078592,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.906488,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.893789,4.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.115652,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.987009,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.956414,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.891763,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.973503,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.967849,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.005635,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.881629,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.915511,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.930373,3.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.985721,1.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.952553,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027199,3.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.948504,1.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.098312,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.110849,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.894264,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.930174,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.015126,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.064958,2.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.895366,1.666700) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.924353,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.989613,4.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.040486,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.096799,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.088074,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.070501,2.333300) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (1.892656,2.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.114393,3.000000) circle[radius=.65pt];
\filldraw[fill=studygray!70!black,draw=white,line width=.15pt] (2.027511,4.333300) circle[radius=.65pt];
\draw[ink,line width=2pt] (2,2.000000) -- (2,3.333300);
\path[fill=white,draw=ink,line width=.45pt] (1.955,2.672222) -- (2,2.782222) -- (2.045,2.672222) -- (2,2.562222) -- cycle;


==> repo/figures/user_study/violin_partimagenet_stats.tex <==
\relax


==> repo/figures/user_study/violin_stats.tex <==
\draw[ink,line width=.45pt] (0,5.13) -- (0,5.20) -- (1,5.20) -- (1,5.13);
\node[anchor=south] at (0.5,5.20) {$^{***}$};
\draw[ink,line width=.45pt] (0,5.48) -- (0,5.55) -- (2,5.55) -- (2,5.48);
\node[anchor=south] at (1,5.55) {$^{***}$};

